Enabling Efficient RDMA-based Synchronous Mirroring of Persistent Memory Transactions

Synchronous Mirroring (SM) is a standard approach to building highly-available and fault-tolerant enterprise storage systems. SM ensures strong data consistency by maintaining multiple exact data replicas and synchronously propagating every update to all of them. Such strong consistency provides fault tolerance guarantees and a simple programming model coveted by enterprise system designers. For current storage devices, SM comes at modest performance overheads. This is because performing both local and remote updates simultaneously is only marginally slower than performing just local updates, due to the relatively slow performance of accesses to storage in today's systems. However, emerging persistent memory and ultra-low-latency network technologies necessitate a careful re-evaluation of the existing SM techniques, as these technologies present fundamentally different latency characteristics compared than their traditional counterparts. In addition to that, existing low-latency network technologies, such as Remote Direct Memory Access (RDMA), provide limited ordering guarantees and do not provide durability guarantees necessary for SM. To evaluate the performance implications of RDMA-based SM, we develop a rigorous testing framework that is based on emulated persistent memory. Our testing framework makes use of two different tools: (i) a configurable microbenchmark and (ii) a modified version of the WHISPER benchmark suite, which comprises a set of common cloud applications. Using this framework, we find that recently proposed RDMA primitives, such as remote commit, provide correctness guarantees, but do not take full advantage of the asynchronous nature of RDMA hardware. To this end, we propose new primitives enabling efficient and correct SM over RDMA, and use these primitives to develop two new techniques delivering high-performance SM of persistent memories.

==> abstract.tex <==
%Enterprise applications require high-availability guarantees.
Synchronous Mirroring (SM) is a standard approach to building highly-available and fault-tolerant enterprise storage systems.
%SM maintains multiple exact data replicas by synchronously propagating every data update to all of them.
%
SM ensures strong data consistency by maintaining multiple exact data replicas and synchronously propagating every update to all of them.
Such strong consistency provides fault tolerance guarantees and a simple programming model coveted by enterprise system designers.
For current storage devices, SM comes at modest performance overheads.  This is because performing both local and remote updates simultaneously is only marginally slower than performing just local updates, due to the relatively slow performance of accesses to storage (e.g., hard drives,
flash-based solid state drives) in today's systems.
However, emerging persistent memory (or storage class memory) and ultra-low-latency network technologies necessitate a careful re-evaluation of the existing SM techniques, as these technologies present fundamentally different latency characteristics compared than their traditional counterparts. In addition to that, existing low-latency network technologies, such as \text{Remote Direct Memory Access (RDMA)}, provide limited ordering guarantees and do not provide durability guarantees necessary for SM. 
 
%In addition to that, given the traditional storage media (i.e., disks) that have been in use for decades, synchronous mirroring comes at very modest performance overhead. That is, remote replica updates are almost as fast as local updates because the remote data update latency was dominated by the disk access latency.

%because of the significant gap between disk and network access latencies,  has always dominated end-to-end latency of synchronous mirroring. because introduces negligible overhead on top of just local updates.

%Moreover, with traditional storage media (e.g., disks) remote data updates were almost as fast as local data updates because the remote data update latency was dominated by the disk access latency.
%So, SM's strong consistency guarantees came at very modest performance overheads.
%However, emerging memory and network technologies necessitate a careful reevaluation of the existing synchronous replication techniques.
%
%
%Even though such strongly consistent systems are known to introduce high overheads, SM is still preferred by enterprise systems for its better fault tolerance and simple programming model.
%
%
%Even though such strongly consistent systems are known to introduce higher overhead compared to weakly consistent systems, most enterprise systems still require SM for the following reasons: (1) The fault tolerance SLAs can only be met with SM (e.g., banking applications that require zero-data-loss) and (2) Given the current technologies, the guarantees of zero-data-loss and simplified programming model far outweigh the performance overheads of SM.
%However, emerging memory and network technologies necessitate a careful reevaluation of the existing synchronous replication techniques.

%This work aims to understand 

%This work aims to provide a detailed study of the performance implications of using \textit{remote direct memory access} (RDMA) in synchronous mirroring of storage class memories.
%\sout{we use an Infiniband test-bed to analyze the latency of memory-level SM. We design and implement a suite of microbenchmarks demonstrate the performance bottlenecks of common RDMA deployments.We find that the state-of-the-art RNIC implementations suffer from poor local DMA performance due to the inefficient PCIe interface, and lack support for \textit{Quality of Service (QoS)}. Second, we develop a cycle-accurate performance model of an RDMA network.}

%\sout{We validate our model using both Infiniband and RoCE and find that the model faithfully reflects the behavior of a typical RDMA network, with an average error of only 1.8\% (6\% max).}
To evaluate the performance implications of RDMA-based SM, we develop a rigorous testing framework that is based on emulated persistent memory.
Our testing framework makes use of two different tools: (i) a configurable microbenchmark and (ii) a modified version of the WHISPER benchmark suite, which comprises a set of common cloud applications, with support for SM over RDMA.
Using this framework, we find that recently proposed RDMA primitives,
such as remote commit, provide correctness guarantees, but do not take full advantage 
of the asynchronous nature of RDMA hardware. To this end, we propose new primitives enabling efficient and correct SM over RDMA, and use these primitives to develop two new techniques delivering high performance SM 
of persistent memories. Overall, we find that our two SM designs outperform the remote commit based design by 1.8x and 2.9x, respectively.

%in a system with storage class memory.
% : (i)~SM with ordered buffering (SM-OB), which leverages the \textit{ordering fence}, \textit{durability fence}, and \textit{RDMA
% write-through} RDMA verbs; and (ii)~SM using non-temporal RDMA writes (SM-DD).

%Overall, we find that our two SM designs slow down persistent memory applications by up to \stanko{\sout{6.3x}NNx and NNx, respectively, compared to NNx using the remote commit design.}
%Based on our findings and for the purpose of providing better support for memory-level SM, we argue for an RNIC design that is tightly integrated with the processor. 

%To gain deep insights into the various factors that determine the performance overheads of SM using storage class memories and \emph{Remote Direct Memory Access} (RDMA). 

%are not suitable for SM due to high performance overheads.
